On the Semantic Latent Space of Diffusion-Based Text-to-Speech Models

The incorporation of Denoising Diffusion Models (DDMs) in the Text-to-Speech (TTS) domain is rising, providing great value in synthesizing high quality speech. Although they exhibit impressive audio quality, the extent of their semantic capabilities is unknown, and controlling their synthesized speech's vocal properties remains a challenge. Inspired by recent advances in image synthesis, we explore the latent space of frozen TTS models, which is composed of the latent bottleneck activations of the DDM's denoiser. We identify that this space contains rich semantic information, and outline several novel methods for finding semantic directions within it, both supervised and unsupervised. We then demonstrate how these enable off-the-shelf audio editing, without any further training, architectural changes or data requirements. We present evidence of the semantic and acoustic qualities of the edited audio, and provide supplemental samples: https://latent-analysis-grad-tts.github.io/speech-samples/.

==> latex/related.tex <==
% \subsection{Text-to-Speech DDMs}
Denoising Diffusion Models (DDMs)~\cite{sohl2015deep} have emerged as a powerful generative tool across a broad variety of tasks and domains. In particular, Text-to-speech (TTS) systems based on diffusion models have shown promising results, offering high-fidelity audio generation with flexible speed-quality trade-offs.
While initial DDMs focused on mel-spectrogram conditioning (e.g., WaveGrad \citep{chen2020wavegrad}, DiffWave \citep{kong2020diffwave}), recent efforts transitioned to direct TTS through models like Diff-TTS \citep{jeong2021diff}, WaveGrad 2 \citep{chen2021wavegrad2}, and Grad-TTS \citep{GradTTS}. Now, advancements like DiffGAN-TTS \citep{liu2022diffgan}, FastDiff \citep{huang2022fastdiff}, and ProDiff \citep{huang2022prodiff} prioritize efficiency and expressiveness, leveraging techniques like adversarial training, efficient convolutions, and knowledge distillation for real-time, high-quality speech synthesis.

Beyond efficiency, researchers have explored diffusion models for controllable and expressive TTS. This includes PromptTTS \citep{guo2023prompttts}, which uses text prompts to control speech style and content, and NaturalSpeech 2 \citep{shen2023naturalspeech}, which leverages speech prompts for zero-shot synthesis. 
PromptTTS 2~\citep{leng2023prompttts} introduces a variation network to capture voice information beyond text prompts, enabling diverse voice generation.

In the image domain, recent research has made strides in understanding and manipulating the latent space of diffusion models for image editing.  
\citet{kwon2022diffusion} discovered a semantically meaningful latent space featuring desirable properties for versatile editing. This discovery was further explored by \citet{Michaeli}, who proposed both unsupervised and supervised methods for identifying semantic directions, allowing for controlled and fine-tuned attribute manipulation. This raise the question whether diffusion-based TTS system also a semantic acoustic latent space to facilitate audio editing. 



% % \subsection{Semantic Directions in Image DDMs}
% % Recent research has made strides in understanding and manipulating the latent space of diffusion models for image editing.
% % \citet{baranchuk2021label} showed that the intermediate activations of diffusion models capture semantic information, making them excellent pixel-level representations for label-efficient semantic segmentation.
% % \citet{tumanyan2023plug} achieved fine-grained control in text-driven image-to-image translation by manipulating spatial features and self-attention within the model. 
% % \citet{kwon2022diffusion} discovered a semantically meaningful latent space ("h-space") featuring desirable properties for versatile editing. This discovery was further explored by \citet{Michaeli}, who proposed both unsupervised and supervised methods for identifying semantic directions, allowing for controlled and fine-tuned attribute manipulation.
% % % \citet{park2023unsupervised} leveraged Riemannian geometry to discover interpretable editing directions in the latent space, achieving disentangled attribute changes, while \citet{gandikota2023concept} derived concept sliders based on low-rank parameter directions for intuitive and controlled image generation. \citet{park2023understanding} analyzed the latent space from a geometric perspective, manipulating local latent basis at specific timesteps for editing and providing insights into its structure and evolution over timesteps.
% % Focusing on score-based models, \citet{wang2023concept} analyzed the way concepts are encoded in disentangled representations, opening up possibilities for manipulating them via algebraic operations.





